Lift, Splat, Map: Lifting Foundation Masks for Label-Free Semantic Scene Completion

Autonomous mobile robots deployed in urban environments must be context-aware, i.e., able to distinguish between different semantic entities, and robust to occlusions. Current approaches like semantic scene completion (SSC) require pre-enumerating the set of classes and costly human annotations, while representation learning methods relax these assumptions but are not robust to occlusions and learn representations tailored towards auxiliary tasks. To address these limitations, we propose LSMap, a method that lifts masks from visual foundation models to predict a continuous, open-set semantic and elevation-aware representation in bird's eye view (BEV) for the entire scene, including regions underneath dynamic entities and in occluded areas. Our model only requires a single RGBD image, does not require human labels, and operates in real time. We quantitatively demonstrate our approach outperforms existing models trained from scratch on semantic and elevation scene completion tasks with finetuning. Furthermore, we show that our pre-trained representation outperforms existing visual foundation models at unsupervised semantic scene completion. We evaluate our approach using CODa, a large-scale, real-world urban robot dataset. Supplementary visualizations, code, data, and pre-trained models, will be publicly available soon.

==> acknowledgements.tex <==
\section{Acknowledgements}
\seclabel{acknowledgements}

\redacted{}

==> tables/cluster_tb.tex <==
\begin{table}[!htbp]
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{|c|rrr|rrr|r|}
\hline
Method              & \multicolumn{3}{c|}{SSM}                & \multicolumn{3}{c|}{TerrainNet}                                     & \multicolumn{1}{c|}{Random Baseline} \\ \hline
Subclass            & \multicolumn{1}{r|}{\% of trials} & \multicolumn{1}{r|}{Precision}      & Recall & \multicolumn{1}{r|}{\% of trials} & \multicolumn{1}{r|}{Precision} & Recall & \textbf{Precision Threshold}         \\ \hline
Light Marb. Tiling  & \multicolumn{1}{r|}{0}            & \multicolumn{1}{r|}{0.15}           & 0.905  & \multicolumn{1}{r|}{0}            & \multicolumn{1}{r|}{0.13}      & 0.851  & \textbf{0.158}                       \\ \hline
Dark Marb. Tiling   & \multicolumn{1}{r|}{0}            & \multicolumn{1}{r|}{0.303}          & 0.889  & \multicolumn{1}{r|}{0}            & \multicolumn{1}{r|}{0.242}     & 0.773  & \textbf{0.325}                       \\ \hline
Porcelain Tile      & \multicolumn{1}{r|}{100}          & \multicolumn{1}{r|}{\textbf{0.306}} & 0.986  & \multicolumn{1}{r|}{0}            & \multicolumn{1}{r|}{0.277}     & 0.969  & \textbf{0.297}                       \\ \hline
Blond Marble Tiling & \multicolumn{1}{r|}{100}          & \multicolumn{1}{r|}{0.041}          & 0.979  & \multicolumn{1}{r|}{0}            & \multicolumn{1}{r|}{0.036}     & 0.921  & \textbf{0.04}                        \\ \hline
Patterned Tile      & \multicolumn{1}{r|}{100}          & \multicolumn{1}{r|}{\textbf{0.281}} & 0.04   & \multicolumn{1}{r|}{0}            & \multicolumn{1}{r|}{0.152}     & 0.879  & \textbf{0.179}                       \\ \hline
Dome Mat            & \multicolumn{1}{r|}{100}          & \multicolumn{1}{r|}{\textbf{0.884}} & 0.417  & \multicolumn{1}{r|}{0}            & \multicolumn{1}{r|}{0.521}     & 0.682  & \textbf{0.557}                       \\ \hline
Door Mat            & \multicolumn{1}{r|}{100}          & \multicolumn{1}{r|}{\textbf{0.647}} & 0.841  & \multicolumn{1}{r|}{100}          & \multicolumn{1}{r|}{0.477}     & 0.86   & \textbf{0.443}                       \\ \hline
Threshold           & \multicolumn{1}{r|}{100}          & \multicolumn{1}{r|}{\textbf{0.682}} & 0.337  & \multicolumn{1}{r|}{0}            & \multicolumn{1}{r|}{0.278}     & 0.639  & \textbf{0.566}                       \\ \hline
Metal Floor         & \multicolumn{1}{r|}{100}          & \multicolumn{1}{r|}{\textbf{0.246}} & 0.738  & \multicolumn{1}{r|}{0}            & \multicolumn{1}{r|}{0.118}     & 0.867  & \textbf{0.176}                       \\ \hline
Other               & \multicolumn{1}{r|}{100}          & \multicolumn{1}{r|}{\textbf{0.386}} & 0.792  & \multicolumn{1}{r|}{0}            & \multicolumn{1}{r|}{0.15}      & 0.355  & \textbf{0.258}                       \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{1em}
\caption{Precision and recall for sub-class prediction, where sub-classes are derived by clustering the penultimate layer's embeddings using Hungarian matching. The baseline represents random precision. Clustering was performed within each super-class}
\label{table:subclass_discovery}
\end{table}

==> tables/object_tb.tex <==
\begin{table}[!htbp]
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{\textbf{Model}} & \multirow{3}{*}{\textbf{mIoU}} & \textbf{Unlabeled}           & \textbf{Car}                 & \textbf{Pedestrian}          & \textbf{Bike}                & \textbf{Scooter}             & \textbf{Tree}                & \textbf{Pole Sign}           & \textbf{Canopy}              & \textbf{Traffic Light}       & \textbf{Bike Rack}           & \textbf{Barrier}             \\ \cline{3-13} 
                                &                                & \textbf{Kiosk Machine}       & \textbf{Dispenser}           & \textbf{Fire}                & \textbf{Plant}               & \textbf{Pole}                & \textbf{Door}                & \textbf{Cone}                & \textbf{Chair}               & \textbf{Bench}               & \textbf{Table}               & \textbf{Trash Can}           \\ \cline{3-13} 
                                &                                & \textbf{Flat Sign}           & \textbf{Aid Kit}             & \textbf{Electronics}         & \textbf{Other}               & \textbf{Cart}                & \textbf{Couch}               & \textbf{Traffic Arm}         & \textbf{Door Switch}         & \textbf{Phone}               & \textbf{Dumpster}            &                              \\ \hline
\multirow{3}{*}{SupCon (ours)}  & \multirow{3}{*}{0.59307}       & \multicolumn{1}{r|}{0.98023} & \multicolumn{1}{r|}{0.83865} & \multicolumn{1}{r|}{0.5817}  & \multicolumn{1}{r|}{0.7456}  & \multicolumn{1}{r|}{0.49008} & \multicolumn{1}{r|}{0.69571} & \multicolumn{1}{r|}{0.51546} & \multicolumn{1}{r|}{0.54428} & \multicolumn{1}{r|}{0.37885} & \multicolumn{1}{r|}{N/A}     & \multicolumn{1}{r|}{0.65281} \\ \cline{3-13} 
                                &                                & \multicolumn{1}{r|}{N/A}     & \multicolumn{1}{r|}{0.68059} & \multicolumn{1}{r|}{0.23165} & \multicolumn{1}{r|}{0.7119}  & \multicolumn{1}{r|}{0.62205} & \multicolumn{1}{r|}{0.64314} & \multicolumn{1}{r|}{0.41794} & \multicolumn{1}{r|}{0.62047} & \multicolumn{1}{r|}{0.74395} & \multicolumn{1}{r|}{0.49929} & \multicolumn{1}{r|}{0.69222} \\ \cline{3-13} 
                                &                                & \multicolumn{1}{r|}{0.4756}  & \multicolumn{1}{r|}{0.25}    & \multicolumn{1}{r|}{N/A}     & \multicolumn{1}{r|}{0.79822} & \multicolumn{1}{r|}{0.63636} & \multicolumn{1}{r|}{0.85096} & \multicolumn{1}{r|}{0.65005} & \multicolumn{1}{r|}{0}       & \multicolumn{1}{r|}{0.65831} & \multicolumn{1}{r|}{N/A}     & \multicolumn{1}{r|}{}        \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{1em}
\caption{Object prediction accuracy (IoU) of ReSS, which employs supervised contrastive loss and focal loss to tackle the challenge of unbalanced labels. N/A indicates that the ground truth label does not exist for that class in the test dataset.}
\label{table:object_scene_completion}
\end{table}
